Variance-adaptive confidence regions for fixed-benchmark binomial mixtures, with application to LLM evaluation

We construct confidence intervals for linear functionals $\theta(F_m)=\int h\,dF_m$ of the empirical law $F_m$ of success probabilities $p_1,\dots,p_m$, from independent counts $c_i\sim\mathrm{Bin}(n,p_i)$, as for a language model run $n$ times per problem. Coverage is at least $1-\alpha$ for every $n$, $m$ and fixed $(p_i)$, simultaneously for all bounded $h$. The variance-adaptive (VA) region tests each candidate mixing law with the conditional variance of the tail counts it implies. This variance is linear in the law, so the region is a linear program, and cell envelopes keep it valid off-grid. Regions calibrated for iid sampling target a super-population law and are conservative for $\theta(F_m)$. With all $n$ tail counts, fixed $n$, continuous $h$ and a grid refined as $m\to\infty$, the identification part of VA's width is first-order worst-case optimal, as for any localization with the same index set. Under a rule fixed before the main comparator runs, VA was narrower than a two-stage plug-in band at every $n$ (median width ratio 0.60 at $n=128$), but not than the asymptotic, pointwise AMARI interval at $n=128$; on real rollout pools it was wider than both pointwise and Bonferroni-adjusted AMARI at $n\le128$. For $P(p>0)$ and pass@$k$ with $k\gg n$ the data support only lower bounds.

==> xref-main.tex <==
\makeatletter
\newlabel{M-sec:intro}{{1}{1}{Introduction}{}{}}
\newlabel{M-sec:related}{{2}{3}{Related work}{}{}}
\newlabel{M-sec:setting}{{3}{4}{Setting, targets and estimand}{}{}}
\newlabel{M-eq:passk-bracket}{{1}{4}{Model and targets}{}{}}
\newlabel{M-tab:Glevel}{{1}{5}{The super-population target $\theta _\delta (G)$, $m=1000$, medians over F1--F5 and three $\delta $ (15 cells per $n$). First column: VA for $\theta _\delta (F_m)$ at level $\alpha $, for reference. ``VA$+$KL'', ``VA$+$EB'', ``VA$+$DKW'': VA at $\alpha /2$ followed by a layer at $\alpha /2$ that covers $\theta (F_m)-\theta (G)$ (Propositions~\ref {S-prop:layer-kl}--\ref {S-prop:layer-dkw}; KL and EB with $J=3$ targets, DKW simultaneous over all monotone targets). ``Best FL'': the narrowest of DKW-Massart, Berk--Jones, KL-Bonf, Hoeff-$k$ and exact-binomial at level $\alpha $; AMARI: Empirikos-faithful, pointwise; oracle: $2z_{0.975}\,\mathrm {sd}_G(h)/\sqrt m$, the interval for an analyst who observes the $p_i$. Last two columns: median ratio of VA$+$KL to the best FL and to AMARI. All comparators were computed on counts drawn under the fixed $F_m$ of the simulation, as a proxy for redrawn $p_i$}{}{}}
\newlabel{M-sec:estimand}{{3.2}{5}{Choice of estimand}{}{}}
\newlabel{M-eq:vargap}{{2}{5}{Tail counts and the variance gap}{}{}}
\newlabel{M-tab:regions}{{2}{6}{Confidence regions compared. All LP regions use the same cells and envelopes, and certified endpoints (except $\chi ^2$, whose LP has auxiliary columns). $L=\log (2|K|/\alpha )$; $K$ is the pre-specified index set of Section~\ref {sec:K}; every LP region also has the sure constraints. ``Unproven'' means finite-sample valid for iid data, with no proof under fixed $p_i$. $^\dagger $Our re-implementation of AMARI (Supplement~\ref {S-supp:comparators})}{}{}}
\newlabel{M-sec:floc}{{3.4}{6}{Generalized F-localization}{}{}}
\newlabel{M-sec:ident}{{3.5}{6}{Identification}{}{}}
\newlabel{M-sec:va}{{4}{7}{The VA region and its coverage}{}{}}
\newlabel{M-lem:bands}{{4.1}{7}{Bands for one tail count}{}{}}
\newlabel{M-prop:twostage}{{4.2}{7}{Two-stage band}{}{}}
\newlabel{M-sec:lp}{{4.3}{8}{The gridded LP}{}{}}
\newlabel{M-eq:lp}{{3}{8}{The gridded LP}{}{}}
\newlabel{M-sec:K}{{4.3}{8}{Choice of $K$}{}{}}
\newlabel{M-thm:coverage}{{4.3}{8}{Finite-sample conditional coverage}{}{}}
\newlabel{M-alg:va}{{1}{9}{Choice of $K$}{}{}}
\newlabel{M-sec:iid}{{5}{10}{Iid-calibrated localizations under fixed $p_i$}{}{}}
\newlabel{M-prop:iid}{{5.1}{10}{Iid calibration under fixed $p_i$}{}{}}
\newlabel{M-eq:factor}{{4}{10}{Iid calibration under fixed $p_i$}{}{}}
\newlabel{M-rem:open-validity}{{5.1}{10}{What remains open}{}{}}
\newlabel{M-sec:width}{{6}{10}{Width theory}{}{}}
\newlabel{M-thm:width}{{6.1}{10}{Width upper bound}{}{}}
\newlabel{M-fig:vargap}{{1}{11}{The variance gap. Ratio of the conditional variance $V_k(F_m)$ to the iid variance $q_k(1-q_k)$ against $k\in K_{\rm geo}$, for the simulation draws of F1--F5 with $m=1000$. F2 (thick) is fitted to Monkey Business}{}{}}
\newlabel{M-cor:oracle}{{6.2}{11}{Comparison with Bonferroni linear certificates}{}{}}
\newlabel{M-thm:id}{{6.3}{12}{Worst-case identification optimality, $K=\{1,\dots ,n\}$}{}{}}
\newlabel{M-rem:cn}{{6.1}{12}{The constant for $h_\delta $}{}{}}
\newlabel{M-sec:separated}{{6.4}{12}{Separated laws}{}{}}
\newlabel{M-prop:realised}{{6.4}{13}{Realised widths of iid-calibrated regions}{}{}}
\newlabel{M-cor:sepA}{{6.5}{13}{Constant-factor gain}{}{}}
\newlabel{M-cor:sepB}{{6.6}{13}{Rate separation in a joint limit}{}{}}
\newlabel{M-op:estimation}{{6.7}{14}{Estimation-term lower bound}{}{}}
\newlabel{M-sec:sim}{{7}{14}{Simulation study}{}{}}
\newlabel{M-sec:sim-design}{{7.1}{14}{Design}{}{}}
\newlabel{M-sec:sim-verdict}{{7.2}{14}{The decision rule and its outcome}{}{}}
\newlabel{M-tab:coverage}{{3}{16}{Coverage evidence at $\alpha =0.05$ (sure constraints in every LP region). Simulation: minimum empirical coverage of $\theta _\delta (F_m)$ over the 45 cells per $n$ (135 in all; AMARI 105, run at $n=512$ for $m=1000$ only), the number of cells whose two-sided 95\% Clopper--Pearson upper bound is below $0.95$, and the replicate range; ``other'' is the minimum over $P(p\ge 0.05)$, $P(p\ge 0.5)$, pass@8 and pass@1024. MB: minimum coverage of $\theta _\delta (\hat p)$ over the eight Monkey Business configurations and the pooled data, all $n$ (AMARI: $n\le 128$). Band: non-coverage of the band event, $R=10^5$ per cell, maximum over cells and number of cells whose Clopper--Pearson lower bound exceeds $\alpha $. For the two-stage band the event is ``the true $F_m$ satisfies the region's constraints''. Full coverage in $R=30$ (or $R=15$) replicates is consistent with true coverage as low as 0.884 (0.782), the two-sided Clopper--Pearson lower bound; these columns check the code. All regions: Table~\ref {S-tab:s4-coverage-full}}{}{}}
\newlabel{M-sec:mb}{{8}{16}{Coverage under resampling from real rollout pools}{}{}}
\newlabel{M-tab:width}{{4}{17}{Median over the simulation cells (F1--F5, $m\in \{250,1000,4000\}$, three $\delta $; 45 cells per $n$, 15 at $n=512$ for AMARI) of the ratio of VA's median width to the comparator's median width for $\theta _\delta (F_m)$, $\alpha =0.05$. Below $1$: VA narrower. Brackets: bootstrap 95\% Monte Carlo intervals of the median (replicates resampled jointly within each $(F,m,n)$ simulation block, across methods and targets). AMARI is the Empirikos-faithful variant; C1--C3 are the comparators of the pre-specified rule (Section~\ref {sec:sim-verdict}). ``Best other localization'' is the narrowest non-VA localization in the cell: KL-Bonf, Hoeff-$k$, Hoeff-cell, both DKW bands, Berk--Jones, EB-DKW, $\chi ^2$, exact-binomial, and the two-stage band with Bernstein or Bennett radius (\VA -iid, a VA ablation, and AMARI are excluded); ``best proven-valid'' is the narrowest of these with a finite-sample proof under fixed $p_i$, that is, all but DKW-Massart, Berk--Jones and $\chi ^2$. The plug-in bootstrap is omitted because it undercovers (Table~\ref {tab:coverage}). All regions: Table~\ref {S-tab:s4-ratio-full}}{}{}}
\newlabel{M-tab:mb-wr}{{5}{18}{Monkey Business, pooled data ($m=1022$ problem--model units), median width of the 95\% interval for $\theta _\delta (\hat p)$, rollouts resampled with replacement, $K_{\rm geo}$. AMARI: Empirikos-faithful (empirical standard error, intersected with the pilot localization), pointwise and at $\alpha /3$; run at $n\le 128$ only. The plug-in bootstrap undercovers (minimum coverage over configurations 0.000, 0.020 and 0.700 at $n=32$, 128 and 512) and is shown for reference}{}{}}
\newlabel{M-sec:pair}{{9}{18}{Illustration: a distilled model and an RL model trained from it}{}{}}
\newlabel{M-tab:e3}{{6}{19}{Distilled model (DeepSeek-R1-Distill-Qwen-1.5B) and RL-from-distilled model (DeepScaleR-1.5B-Preview) on the counts of \citet {yang2026crossovers}, $m=1060$, $n=128$; sure constraints in every LP region. Marginal 95\% intervals (certified endpoints) and the Bonferroni difference (each marginal at $\alpha /2$). $^*$Excludes 0. AMARI: Empirikos-faithful, pointwise and Bonferroni-adjusted over the eight targets ($\alpha /8$). The plug-in bootstrap targets the observed-count functional $m^{-1}\sum _ih(c_i/n)$, has no coverage guarantee for $\theta (F_m)$ and undercovered in the simulations. AMARI is intersected with a pilot DKW localization at the fixed level 0.01, not adjusted for multiplicity; for $P(p\ge 0.5)$ the pilot interval binds, so the pointwise and $\alpha /8$ intervals coincide. AMARI's pass@$k$ intervals use point evaluation on a finite node set. All regions and the targets $\theta _{0.02}$, $P(p\ge 0.05)$, pass@256 and $P(p>0)$: Table~\ref {S-tab:e3-all}}{}{}}
\newlabel{M-sec:disc}{{10}{20}{Discussion}{}{}}
\newlabel{M-fig:forest}{{2}{21}{Distilled and RL-from-distilled models on the counts of \citet {yang2026crossovers}. Left: marginal 95\% intervals (faint: distilled; solid: RL) for VA, the two-stage band, Berk--Jones and AMARI (pointwise). Right: Bonferroni intervals for the difference RL$-$distilled; the star marks the one interval that excludes zero (VA, $P(p\ge 0.5)$)}{}{}}
\newlabel{M-tab:which}{{7}{22}{When to use which method}{}{}}
\newlabel{M-sec:decl}{{10}{23}{Declarations}{}{}}
\newlabel{M-end:body}{{10}{23}{Use of AI assistance}{}{}}
\makeatother

